The Facebook Algorithm's Active Role in Climate Advertisement Delivery

Communication strongly influences attitudes on climate change. Within sponsored communication, high spend and high reach advertising dominates. In the advertising ecosystem we can distinguish actors with adversarial stances: organizations with contrarian or advocacy communication goals, who direct the advertisement delivery algorithm to launch ads in different destinations by specifying targets and campaign objectives. We present an observational (N=275,632) and a controlled (N=650) study which collectively indicate that the advertising delivery algorithm could itself be an actor, asserting statistically significant influence over advertisement destinations, characterized by U.S. state, gender type, or age range. This algorithmic behaviour may not entirely be understood by the advertising platform (and its creators). These findings have implications for climate communications and misinformation research, revealing that targeting intentions are not always fulfilled as requested and that delivery itself could be manipulated.

==> data-and-code.tex <==
\section*{Data and Code Availability}
All data, code for stimuli selection and analysis notebooks are available on XXX.

==> significance.tex <==
\significancestatement{Sponsored climate change communication has been shown to polarize individuals and groups in the United States. Conventional knowledge about actors who polarize the climate discourse on social media has been restricted to climate contrarian and climate advocacy corporations, organizations, and individuals. We show that advertising algorithms play a significant role in climate change polarization. Using user profiling, algorithms determine target audience for an advertisement on the basis of its content, and independent of advertiser preferences. Climate change advertisements can therefore be differently priced and delivered to different target demographics. Such inconsistencies in the delivery can have implications for climate communication, and climate dis(mis)information research. We call attention to the need for more transparency and regulation around climate change advertising.}
